Finding Cut-Offs in Leaderless Rendez-Vous Protocols is Easy

In rendez-vous protocols an arbitrarily large number of indistinguishable finite-state agents interact in pairs. The cut-off problem asks if there exists a number $B$ such that all initial configurations of the protocol with at least $B$ agents in a given initial state can reach a final configuration with all agents in a given final state. In a recent paper (Horn and Sangnier, CONCUR 2020), Horn and Sangnier proved that the cut-off problem is decidable (and at least as hard as the Petri net reachability problem) for protocols with a leader, and in EXPSPACE for leaderless protocols. Further, for the special class of symmetric protocols they reduce these bounds to PSPACE and NP, respectively. The problem of lowering these upper bounds or finding matching lower bounds was left open. We show that the cut-off problem is P-complete for leaderless protocols and in NC for leaderless symmetric protocols. Further, we also consider a variant of the cut-off problem suggested in (Horn and Sangnier, CONCUR 2020), which we call the bounded-loss cut-off problem and prove that this problem is P-complete for leaderless protocols and NL-complete for leaderless symmetric protocols. Finally, by reusing some of the techniques applied for the analysis of leaderless protocols, we show that the cut-off problem for symmetric protocols with a leader is NP-complete, thereby improving upon all the elementary upper bounds of (Horn and Sangnier, CONCUR 2020).

==> bounded-leftover-threshold.tex <==
\begin{definition}
A conservative Petri net has a bounded-loss threshold,
if there are constants $L$ and $n_0$,
such that for each $n>n_0$
$n\times p_i$ can reach some marking with
ot most $L$ tokens
outside $p_f$.
\end{definition}

\begin{theorem}
There is a polynomial algorithm deciding whether a conservative
Petri net has a bounded-loss threshold.
\end{theorem}

\begin{proof}

We start by describing an algorithm.

Step 1. \textit{Reachability analysis}.

We keep a set of proven-reachable places. 
A place is reachable if 
it can be covered given 
a large enough
initial marking. 

The initial place $p_i$ is proven-reachable by definition.
Every output place of a transition with proven-reachable inputs 
is proven-reachable.
In a single pass over all transitions we can either add one more place,
or verify that all reachable places have been proven reachable.
Thus we can find all reachable places in polynomial time.
It is clear that all the unreachable places can be removed.

We call a transition reachable if all its inputs are reachable.

Step 2. \textit{Linear analysis}.

If a bounded-loss threshold exists,
normalising the transition firing counts would yield
as limit points
rational solutions to the marking equation
moving one token from the initial state to the final state,
and using only reachable transitions.

This is a system of rational linear equations which can be solved
in polynomial time.
If there is no solution, bounded-loss threshold property cannot hold.
Otherwise we will use the solution to proof the bounded-loss threshold.

Step 3. \textit{Constructing one firing sequence}.

We proceed to construct one firing sequence covering the final place.
We multiply the rational solution ofthe marking equation 
by a large enough integer multiplier to obtain an integer solution moving  more tokens.
We use reachability proofs 
to construct an accelerated firing sequence putting enough tokens
in each reachable state
to fire this intteger solution in parallel.
This puts some token into the final place, 
and leaves a lot of tokens elsewhere.

Step 4. \textit{Scaling the construction}.

We now notice that after firing the integer solution
only the token counts in the initial and the final places change.
If we have enough tokens in the initial place to repeat 
the parallel firing 
(all other reachable places have enough tokens by assumption),
we can perform the parallel firing again.
Repeat this asd many times as possible.

Consider a large enough initial marking and perform 
the prefilling of reachable places
the repeated parallel firing of the integer solution.
The reachable places except the initial and the final one
will have some number of tokens independent of the initial configuration size.
The initial state will have at most the number of tokens
one less than the norm of the integer solution.
All the remaining tokens are in the final place.
Thus the constructed family of firing sequences
proves bounded-loss threshold property.

\textit{Conclusion}.


We have shown that computing reachable places and transitions,
and computing a rational solution of the marking equation, 
can be done in polynomial time.
We have also shown that both steps succeed iff the bounded-loss 
threshold property holds.
thus bounded-loss threshold property can be verified in polynomial time.

\end{proof}

\begin{corollary}
If a conservative Petri net has a sublinear-loss threshold,
it has a bounded-loss threshold.
\end{corollary}

\begin{theorem}
Deciding whether a conservative
Petri net has a bounded-loss threshold
is $P$-hard.
\end{theorem}

\begin{proof}
The construction for the existence of a threshold  provides a net where 
$fin$ can be reached
either by all the agents or by none of them.
For such a net allowing a bounded loss does not change the problem,
and hence $P$-hardness still holds.
\end{proof}


==> fracas-haddad_-_Copy.tex <==
Similar to the case of acyclic net systems, we would like to provide
a characterization of net systems admitting a cut-off and then
use this characterization to derive a polynomial time algorithm.
Unfortunately, in general net systems there is no 
characterization of reachability akin to Lemma~\ref{lem:acyclic} for
acyclic systems. 
To this end, we prove two intermediate lemmas to help us come 
up with a characterization for cut-off admissible net systems in the general
case. We believe that these two lemmas could be of independent interest in their
own right. Further, the proofs of both the lemmas are provided so that
it will enable us later on to derive a bound on the cut-off for 
net systems.

\subsection{Lifting lemma (Working title)}

<<<<<<< HEAD
The lifting lemma shows that, given a Petri net system $(\net, M, M')$, the existence of a number $n  \geq 1$ 
such that $n M \reachN{*} n M'$ can be decided in polynomial time, and that if such an $n$ exists then it can be chosen 
of size $O(2^{|\net|})$. The first part follows immediately from a result by Fraca and Haddad showing that the reachability problem for continuous Petri nets is polynomial. We start by recalling this result.

\subsubsection{Reachability in continuous Petri nets.} Petri nets can be given a \emph{continuous semantics} \cite{}, in which
markings are continuous multisets; we call them \emph{continuous markings}. 
A continuous marking $M$ enables transition $t$ \emph{with factor $\lambda \in \qnz$} if
$M(p) \ge \lambda \cdot Pre[p,t]$ for every place $p$; we also say that $M$ enables $\lambda t$.
If $M$ enables $ \lambda t$,  then $\lambda t$ can fire or occur, leading to a new marking $M'$ given 
by $M'(p) = M(p) + \lambda \cdot \incidence[p,t]$ for every $p \in P$. We denote this by $M \reachQ{\lambda t} M'$,
and say that $M'$ is reached from $M$ by firing $\lambda t$. A \emph{continuous firing sequence} is any sequence of transitions $\sigma = \lambda_1 t_1, \lambda_2 t_2,\dots, \lambda_k t_k \in (\qnz \times T)^*$. 
We let $M \reachQ{\sigma} M'$ denote that there exist continuous markings $M_1,\dots,M_{k-1}$
such that $M \reachQ{\lambda_1 t_1} M_1 \reachQ{\lambda_2 t_2} M_2 \ldots \reachN\lambda_{k-1} M_{k-1}
\reachN{t_k} M'$. Further, $M \reachQ{*} M'$ denotes that $M \reachQ{\sigma} M'$ for some continuous firing sequence 
$\sigma$.

The \emph{Parikh image} of $\sigma= \lambda_1 t_1, \lambda_2 t_2,\dots, \lambda_k t_k \in (\qnz \times T)^*$
is the vector $\parikh{\sigma} \in \qnz^T$  where $\parikh{\sigma}[t] = \sum_{i= 1}^k  \delta_{i,t} \lambda_i$,
where $\delta_{i,t} = 1$ if $t_i = t$ and $0$ otherwise.  If $M \reachQ{\sigma} M'$ then$\parikh{\sigma}$ is a solution of the marking equation  over $\qnz^T$, but the converse does not hold.  In \cite{FracaH15}, Fraca and Haddad  strengthen this necessary condition to make it also sufficient, and use the resulting characterization to derive a polynomial algorithm.

\begin{theorem}\cite{FracaH15}
\label{thm:reachQ}
Let $(\net,M,M')$ be a Petri net system.
\begin{itemize}
\item $M \reachQ{\sigma} M'$ if{}f $\parikh{\sigma}$ is a solution of the marking equation  over $\qnz^T$, and there exist continuous firing sequences $\tau$ and $\tau'$ such that $\support{\tau} = \support{\sigma} = \support{\tau'}$, $M \reachQ{\tau}$,  and $ \reachQ{\tau'} M'$.
\item  It can be decided in polynomial time if $M \reachQ{*} M'$ holds.
\end{itemize}
\end{theorem}

\subsubsection{The Lifting Lemma.}  It follows easily from the definitions that $n M \reachN{*} n M'$ holds for some $n \geq 1$ if{}f $M \reachQ{*} M'$.
Indeed, if $M \reachQ{\sigma} M'$ for some $\sigma = \lambda_1 t_1, \lambda_2 t_2,\dots, \lambda_k t_k \in (\qnz \times T)^*$, then $nM \reachQ{n\sigma} nM'$ where $n$ is the smallest number such that $n \lambda_i \in \N$ for every $1 \leq i \leq k$, and $n \sigma = t_1^{n \lambda_1} t_2^{n \lambda_2} \dots t_k^{n \lambda_k}$. So Theorem \ref{thm:reachQ} immediately implies that the the existence of  $n  \geq 1$  such that $n M \reachN{*} n M'$ can be decided in polynomial time. While a bound on the size of $n$ is implicit in the proof of Theorem \ref{thm:reachQ}, it is quite hidden. The Lifting lemma makes We make it explicit by means of two lemmas proved in the appendix. 

\begin{restatable}{lemma}{LiftingLemmaInFull}
\label{lem:fh}
Let $(\net,M,M')$ be a Petri net system such that $M \reachQ{\sigma} M'$ for some continuous firing sequence $\sigma \in (\qnz \times T)^*$.
Let $m$ be the number of transitions in $\supp{\sigma}$, and let $\beta = (W+1)^m$. Let $k$ be the smallest natural number such that $k \cdot \parikh{\sigma} \in \nn^T$, and let $\ell$ be $\|\parikh{\sigma}\|$. Then, there exists a firing sequence $\tau \in T^*$ 
=======
Petri nets can be given a \emph{continuous semantics} \cite{}. In this semantics,
markings are continuous multisets (we call them continuous markings)

Let $\net$ be a net where $\net = (P,T,Pre,Post)$, 
$\incidence$ is its incidence matrix and 
$W$ is the maximum absolute value appearing in the matrices $Pre$ 
and $Post$.
In this section, we show how to \emph{lift} a firing sequence leading from $M$ to $M'$ 
in the continuous semantics, to a firing sequence leading from $nM$ to $nM'$ in the discrete semantics for 
some $n \in \nn$. The proof also provides a exponential upper bound on $n$. More formally, 
the main result of this subsection is the following:

\begin{lemma}[Lifting lemma]
Let $(\net,M,M')$ be a Petri net system. If $M \reachQ{*} M'$, then there exists $n \in 2^{|\net|^{O(1)}}$ such that 
$nM \reachN{*} nM'$.
\end{lemma}

To prove the lifting lemma, we need a number of auxiliary lemmas, 
the first of which is the following:

\begin{lemma}\label{lem:saturation}
	Let $M_0$ be a marking such that $M_0 \reachQ{\sigma}$ for
	some firing sequence $\sigma$. Let $m$ be the size of $\supp{\sigma}$. %and let 
	%$W =  \max \{\|Pre[p,t]\| \mid t \in \supp{\sigma}, p \in \preset{t} \}$.
	There exists a firing sequence  $$\left( (W +1)^m \cdot M_0 \right) \xrightarrow{\tau} M$$
	\noindent such that $\supp{\tau} = \supp{\sigma}$, $|\tau| \leq 2 (W +1)^m$ and $M(p) > 0$ 
	for every $p \in \supp{M_0} \cup \pre{\post{\supp{\sigma}}}$
\end{lemma}

\begin{proof}
	Let $t_1, t_2, \ldots, t_m$ be the transitions of $\supp{\sigma}$, sorted according to the order of
	their first occurrence in $\sigma$.   Let $\beta_0 = 1$, $\beta_i = (W+1)^{i}$ for every $i \in \{1, \ldots, m\}$, and define the sequence 
	$$\tau_0 = \epsilon$$
	$$\tau_i = t_1^{\beta_{i-1}} t_{2}^{\beta_{i-2}} \cdots t_i^{\beta_0} \ $$
	By the definition of $\beta_i$ we have $|\tau_i| \leq 2 (W +1)^i$. We prove for every $i \geq 0$ that 
	$$(\beta_i \cdot M_0) \xrightarrow{\tau_i} M_i$$
	\noindent for some marking $M_i$ such that $M_i(p) > 0$
	for every $p \in \supp{M_0} \cup \pre{\post{\supp{\tau_i}}}$.
	Since $\supp{\tau_m} = \supp{\sigma}$, the claim of the lemma
	would then follow.
	The proof is by induction on $i$.
	
	\medskip\noindent\textbf{Basis: $i=0$.} Then $\beta_i = 1$ and the result follows from $M_0 \xrightarrow{\epsilon} M_0$.
	
	%\medskip\noindent\textbf{Basis: $m=1$.} Then $\sigma$ only contains $t_1$. Since $M_0$ enables $\sigma$, it enables $t_1$. Since $\beta(1) = \alpha + 1$ and $t_1$ takes at most $\alpha$ tokens from each of its input places, we have
	%
	%$$(\beta(1) \cdot M_0)  \reachN{t_1} M_1$$
	%
	%\noindent where the marking $M_1$ marks every place marked at $M_0$ and all input and output places of $t_1$. 
	
	\medskip\noindent\textbf{Induction Step:  $i \geq 1$.} Since $M_0$ enables $\sigma$, it also enables some 
	prefix of $\sigma$ with support $t_1, \ldots, t_{i-1}$. By induction hypothesis,
	$$(\beta_{i-1} \cdot M_0) \xrightarrow{\tau_{i-1}} M_{i-1}$$
	\noindent  where $M_{i-1}(p) > 0$ for every $p \in \supp{M_0} \cup \pre{\post{\supp{\tau_{i-1}}}}$ . Since $\beta_i = (W +1) \beta_{i-1}$ we have
	$$(\beta_i \cdot M_0)  \xrightarrow{\tau_{i-1}^{W +1}} \; ((W +1) \cdot M_{i-1})$$
	
	\noindent Since  $M_0 \reachQ{\sigma}$ and $t_i$ appears in $\sigma$,
	it follows that for every place $p \in \pre{t_i}$,
	%So every place in $\pre{t_i}$ 
        has at least $(W + 1)$ tokens at the marking $(W+1) \cdot M_{i-1}$. It then follows that $(W+1) \cdot M_{m-1} \xrightarrow{t_i} M_i$ for some marking $M_i$ 
	such that $M_i(p) > 0$ for every $p \in \supp{M_0} \cup 
	\pre{\post{\{t_1,\dots,t_i\}}}$.
\end{proof}




%\begin{lemma}\label{lem:saturation}
%Let $(N, M_0)$ be a Petri net and let $M_0 \reachQ{\sigma}$. Let $m$ be the number of transitions of $\supp{\sigma}$, and let 
%$\alpha =  \max \{ W(p, t) \mid t \in \supp{\sigma}, p \in \preset{t} \}$.
%There exists a firing sequence  $$\left( (\alpha +1)^m \cdot M_0 \right) \reachN{\tau} M$$
%\noindent such that $|\tau| \leq 2 (\alpha +1)^m$ and $M$ marks every place marked at $M_0$ and every input and output place of $\supp{\sigma}$. 
%\end{lemma}

%\begin{proof}
%Let $t_1, t_2, \ldots, t_m$ be the transitions of $\supp{\sigma}$, sorted according to the order of
%their first occurrence in $\sigma$.   Let $\beta(i) = (\alpha+1)^{i}$ for every $i \in \{1, \ldots, m\}$, and define the sequence 
%$$\tau_m = t_1^{\beta(m-1)} t_{2}^{\beta(m-2)} \cdots t_m^{\beta(0)} \ .$$
%Further, let $\beta(0)=0$ and $\tau_0 = \epsilon$. By the definition of $\beta(i)$ we have $|\tau| \leq 2 (\alpha +1)^m$. We prove for every $m \geq 0$ that 
%$$(\beta(m) \cdot M_0) \reachN{\tau_m} M_m$$
%\noindent for some marking $M_m$ that marks every place marked at $M_0$ and every input and output place of $\supp{\tau_m}$. Since $\supp{\tau_m} = \supp{\sigma}$, we are done.
%The proof is by induction on $m$.

%\medskip\noindent\textbf{Basis: $m=0$.} Then $(\alpha +1)^m = 1$ and $\supp{\sigma} = \emptyset$, and the result follows from $M_0 \reachN{\epsilon} M_0$.

%%\medskip\noindent\textbf{Basis: $m=1$.} Then $\sigma$ only contains $t_1$. Since $M_0$ enables $\sigma$, it enables $t_1$. Since $\beta(1) = \alpha + 1$ and $t_1$ takes at most $\alpha$ tokens from each of its input places, we have
%%
%%$$(\beta(1) \cdot M_0)  \reachN{t_1} M_1$$
%%
%%\noindent where the marking $M_1$ marks every place marked at $M_0$ and all input and output places of $t_1$. 

%\medskip\noindent\textbf{Step:  $m \geq 1$.} Since $M_0$ enables $\sigma$, it also enables some 
%prefix of $\sigma$ with support $t_1, \ldots, t_{m-1}$. By induction hypothesis,
%$$(\beta(m-1) \cdot M_0) \reachN{\tau_{m-1}} M_{m-1}$$
%\noindent  for some marking $M_{m-1}$ that marks every place marked at $M_0$ and every input and output place of  $t_1, t_2, \ldots, t_{m-1}$.  Since $\beta(m) = (\alpha +1) \beta(m-1)$ we have

%$$(\beta(m) \cdot M_0)  \reachN{\tau_{m-1}^{\alpha +1}} \; ((\alpha +1) \cdot M_{m-1})$$

%\noindent Since  $M_0 \reachQ{\sigma}$ and $t_m$ appears in $\sigma$, every input place of $t_m$ is marked at $M_0$ or is an output place of at least one of $t_1, \ldots, t_{m-1}$. So every place 
%in the preset of $t_m$ has at least $(\alpha + 1)$ tokens at $M_{i-1}$. It follows $M_{m-1} \reachN{t_m} M_m$ for some marking $M_m$ that marks every place marked at $M_0$ and every input and output place of $t_1, \ldots, t_{m}$.  
%\end{proof}






\begin{lemma}\label{lem:iter}
	Let $M_0$ and $M$ be markings and let $\sigma$ be a firing sequence such that $M_0 \xrightarrow{\sigma}$,
	$\xrightarrow{\sigma} M$, and $n \parikh{\sigma}$ is a solution of the marking equation for some $n \ge 0$.
	Then $M_0 \xrightarrow{\sigma^n} M$.
\end{lemma}
\begin{proof}
	TBD. 
\end{proof}



%\begin{lemma}
%\label{lem:iter}
%Let $(N, M_0)$ be a Petri net. If $M_0 \reachN{\sigma}$, $\reachN{\sigma} M$, and $M = M_0 + \inc{N} \cdot n \cdot \vec{\sigma}$ for some $n \geq 0$, then $M_0 \reachN{\sigma^n} M$.
%\end{lemma}
%\begin{proof}
%TBD.
%\end{proof}

\begin{proposition}\label{prop:easy}
Suppose $M$ is a marking and $\sigma$ is a firing sequence
such that $M(p) \ge W \cdot \parikh{\sigma}(t)$ for every $t \in \supp{\sigma}$ and for every $p \in \pre{t}$. Then $M \xrightarrow{\sigma}$.
\end{proposition}

\begin{proof}
Very easy induction on $\sum_{t \in T} \parikh{\sigma}(t)$.
\end{proof}


\begin{lemma}
\label{lem:fh}
Let $M_0$ and $M$ be markings such that $M_0 \reachQ{\sigma} M$
for some firing sequence $\sigma$.
Let $m$ be the size of $\supp{\sigma}$, $\beta = (W+1)^m$, let
$k$ be the smallest natural number such that $k \cdot \parikh{\sigma} \in \nn^T$, and let $\ell$ be $\|\parikh{\sigma}\|$. Then, there exists a sequence $\tau$ 
>>>>>>> 4352244b6bd7ec5dad0024543ede5453f2c15d05
such that $\supp{\tau} = \supp{\sigma}$ and
%$|\tau| \leq 4 Wk \ell + 16 W k^2  \ell^2$ and
$$\left( 16 W (W+1)^{2m} k \ell \cdot M_0 \right) \xrightarrow{\tau} \left( 16 W (W+1)^{2m} k \ell \cdot M \right)$$
\end{restatable}

<<<<<<< HEAD
\begin{restatable}{lemma}{LiftingLemmaShort}\textbf{\textrm{(Lifting Lemma)}}
\label{lem:fhshort}
Let $(\net,M,M')$ be a Petri net system. If $M~\reachQ{*}~M'$, then there exists $n \in O(2^{|\net|})$ such that 
$nM \reachN{*} nM'$.
\end{restatable}
=======
\subsubsection{Second firing sequence: }
By construction of $\tau_1$ and $\tau_2$ we have that
$|\tau_1|, |\tau_2| \le 2\beta$. It follows then that
$\|\tau_1\| + \|\tau_2\| \le 4\beta$. Once again by construction
of $\tau_1$ and $\tau_2$ we have that $\supp{\tau_1} = \supp{\tau_2} = \supp{\sigma}$. Further by construction of the number $k$,
it follows that all the non-zero components of $4k\beta \parikh{\sigma}$
are at least $4\beta$. Hence, if we define 
\begin{equation}
\label{eq:fh1.5}
v := 4 \beta k \cdot \parikh{\sigma} - (\parikh{\tau}_1 + \parikh{\tau}_2) 
\end{equation}
then $v$ is a non-negative integer vector.

Let $\tau_3$ be any firing sequence such that $\parikh{\tau_3} = v$.
We claim that $\gamma L_1 \xrightarrow{\tau_3}, \xrightarrow{\tau_3} \gamma L_2$
and $\gamma L_2 = \gamma L_1 + \incidence \cdot (\gamma \cdot v)$. Notice that if this claim
is true, then by Lemma~\ref{lem:iter} we have that
$\gamma L_1 \xrightarrow{\tau_3^{\gamma}} \gamma L_2$ and then
the second part of equation~\ref{eq:three-parts} will also be done,
thereby making the proof complete.\\


All that is left to prove are the three claims. 
As remarked at the end of the first part of the construction,
notice that $(\gamma \cdot L_1)(p) \ge \gamma$ for every $p \in \pre{\post{\supp{\sigma}}}$. Since $\parikh{\tau_3} = v$, 
by equation~\ref{eq:fh1.5} notice
that $\supp{\tau_3} \subseteq \supp{\sigma}$
and $W \cdot \|\parikh{\tau_3}\| \le W \cdot 4\beta k \cdot \|\parikh{\sigma}\| \le W \cdot 4\beta k \ell = \gamma$.
Hence it follows that $(\gamma \cdot L_1)(p) \ge W \|\parikh{\tau_3}\|$ for every $p \in \pre{\post{\supp{\tau_3}}}$.
Applying proposition~\ref{prop:easy}, we get that $\gamma \cdot L_1 \xrightarrow{\tau_1}$.

By the same argument applied to the reverse net $\net^{-1}$,
we can get that $\gamma \cdot L_2 \xrightarrow{\tau_2^{-1}}$
in the reverse net $\net^{-1}$, hence leading to 
$\xrightarrow{\tau_2} \gamma \cdot L_2$.

Finally, notice that 
$$\begin{array}{lclrr}
L_2 & = & 4 k \beta \cdot  M - \incidence \cdot \parikh{\tau_2} & \ \qquad \ & \mbox{($L_2 \xrightarrow{\tau_2} 4k\beta \cdot M$)}\\
& = & 4 \beta k \cdot  M_0 + \incidence \cdot 4 \beta k \cdot \parikh{\sigma}  - \incidence  \cdot \parikh{\tau_2} &  & \mbox{($M_0 \reachQ{\sigma} M$)}\\
& = & L_1 - \incidence \cdot \parikh{\tau_1} + \incidence \cdot 4 \beta k \cdot \parikh{\sigma} - \incidence \cdot \parikh{\tau_2}  & & \mbox{($4k\beta \cdot M_0 \xrightarrow{\tau_1} L_1$)}\\
& = &  L_1 + \incidence \cdot (4 \beta k \cdot \parikh{\sigma} - (\parikh{\tau_1} + \parikh{\tau_2})) \\
& = & L_1 + \incidence \cdot v & & \mbox{(Equation~\ref{eq:fh1.5})}\\
\end{array}$$
and so $\gamma \cdot L_2 = \gamma \cdot L_1 + \incidence \cdot (\gamma \cdot v)$. Since all the three claims have been proven, the proof is now complete and we have established the desired run.

\end{proof}

Finally, we get the proof of the lifting lemma.
\begin{lemma}[Lifting lemma]~\label{lem:lifting-lemma}
	Suppose $M$ and $M'$ are markings of $\net$ such that
	$M \xrightarrow[\qn]{*} M'$. Then 
        there exists $n \in 2^{|\net|^{O(1)}}$ such that 
	$nM \xrightarrow{*} nM'$.
\end{lemma}

\begin{proof}
	Suppose $M \xrightarrow[\qn]{*} M'$ for some $\sigma'$.
	By~(\cite{BFHH17}, Proposition 3.2), there is a formula $\phi(M,M',\vect)$ in the existential
	theory of linear rational arithmetic whose size is linear in the size of the net $\net$ such that $\phi(M,M',\by)$
	is true iff there exists $\sigma$ such that $\parikh{\sigma} = \by$
	and $M \xrightarrow[\qn]{\sigma} M'$.
	By~(\cite{Sontag85}, Lemma 3.2) if an formula in existential theory of
	linear rational arithmetic is satisfiable, then it 
	is satisfiable by a solution which can be described using 
	a polynomial number of bits in the size of the formula.
	Hence, if there is a solution to $\phi(M,M',\vect)$,
	then there is a solution which is at most $2^{|\net|^{O(1)}}$.
	Combining all this, we get that there is a $\sigma$
	such that the numerator and denominator of every entry of $\parikh{\sigma}$ is at most 
	$2^{|\net|^{O(1)}}$ and $M \xrightarrow[\qn]{\sigma} M'$.
	
	Notice that the smallest natural number $k$ such that
	$k \cdot \parikh{\sigma} \in \nn^T$ is at most the
	least common multiple of the denominators of all
	the numbers in $\parikh{\sigma}$.
	Since the size of $\parikh{\sigma}$ is bounded by $2^{|\net|^{O(1)}}$,
	it follows then that $k$ and $\|\parikh{\sigma}\|$ are bounded by 
	$2^{|\net|^{O(1)}}$ as well.
	Since the size of $\supp{\sigma}$ is at most the number of transitions
	$|T|$, if we let $W$ be the maximum absolute value appearing in the matrices $Pre$ and $Post$, then $(W+1)^{\supp{\sigma}}$
	is once again at most $2^{|\net|^{O(1)}}$.
	
	Applying Lemma~\ref{lem:fh} we now get that there exists
	$n \in 2^{|\net|^{O(1)}}$ such that $nM_0 \xrightarrow{*} nM$.
\end{proof}

%\begin{lemma}
%\label{lem:fh}
%Let $(N, M_0)$ be a Petri net with $m$ transitions and let $M_0 \reachQ{\sigma} M$. 
%Let $k$ be the smallest natural number such that $k \cdot \sigma$ is an integer sequence, and let $\ell$ be the sum of the components of $\vec{\sigma}$. There exists a sequence $\tau$ such that
%$|\tau| \leq 4 \alpha \beta  \ell + 16 \alpha \beta^2  \ell^2$ and
%$$\left( 16 \alpha (\alpha +1)^{2m} k \ell \cdot M_0 \right) \reachN{\tau} \left( 16 \alpha (\alpha +1)^{2m} k \ell \cdot M \right) \;\; .$$
%\end{lemma}
>>>>>>> 4352244b6bd7ec5dad0024543ede5453f2c15d05




%\subsubsection{Acknowledgements.} \small{The work of the
%second and fifth author has received funding from the European Research
%Council (ERC) under the European Union's Horizon 2020 research and
%innovation programme under grant agreement No 787367 (PaVeS).}

